Smooth Indirect Solution Method for State-constrained Optimal Control Problems with Nonlinear Control-affine Systems

This paper proposes a new indirect solution method for solving state-constrained optimal control problems by revisiting the well-established optimal control theory and addressing the long-standing issue of discontinuous control and costate due to pure state inequality constraints. It is well-known that imposing pure state path constraints in optimal control problems introduces discontinuities in the control and costate, rendering the classical indirect solution methods ineffective to numerically solve state-constrained problems. This study re-examines the necessary conditions of optimality for a class of state-constrained optimal control problems, and shows the uniqueness of the optimal control input that minimizes the Hamiltonian on constrained arcs. This analysis leads to a unifying form of optimality necessary conditions and thereby address the issue of discontinuities in control and costate by modeling them via smooth functions, transforming the originally discontinuous problems to smooth two-point boundary value problems (TPBVPs), which can be readily solved by existing nonlinear root-finding algorithms. The proposed solution method is shown to have favorable properties, including its anytime algorithm-like property, which is often a desirable property for safety-critical applications, and numerically demonstrated by an optimal orbital transfer problem.

==> bbl.tex <==
\begin{thebibliography}{10}

\bibitem{Hartl1995}
R.~F. Hartl, S.~P. Sethi, and R.~G. Vickson, ``A {{Survey}} of the {{Maximum
  Principles}} for {{Optimal Control Problems}} with {{State Constraints}},''
  {\em SIAM Review}, vol.~37, pp.~181--218, June 1995.

\bibitem{Bryson1975}
A.~E. Bryson and Y.-C. Ho, {\em Applied {{Optimal Control}}}.
\newblock {Routledge}, 1975.

\bibitem{Speyer1968}
J.~L. Speyer and A.~E. Bryson, ``Optimal programming problems with a bounded
  state space.,'' {\em AIAA Journal}, vol.~6, pp.~1488--1491, Aug. 1968.

\bibitem{Bock1984}
H.~G. Bock and K.~J. Plitt, ``A {{Multiple Shooting Algorithm}} for {{Direct
  Solution}} of {{Optimal Control Problems}}*,'' {\em IFAC Proceedings
  Volumes}, vol.~17, pp.~1603--1608, July 1984.

\bibitem{Hargraves1987a}
C.~R. Hargraves and S.~W. Paris, ``Direct {{Trajectory Optimization Using
  Nonlinear Programming}} and {{Collocation}},'' {\em Journal of Guidance,
  Control, and Dynamics}, vol.~10, no.~4, pp.~338--342, 1987.

\bibitem{Szmuk2020}
M.~Szmuk, T.~P. Reynolds, and B.~A{\c c}{\i}kme{\c s}e, ``Successive
  {{Convexification}} for {{Real-Time Six-Degree-of-Freedom Powered Descent
  Guidance}} with {{State-Triggered Constraints}},'' {\em Journal of Guidance,
  Control, and Dynamics}, vol.~43, pp.~1399--1413, Aug. 2020.

\bibitem{Nocedal2006b}
J.~Nocedal and S.~J. Wright, ``Interior-{{Point Methods}} for {{Nonlinear
  Programming}},'' in {\em Numerical {{Optimization}}}, pp.~563--597, {New
  York}: {Springer New York}, 2006.

\bibitem{Mao2016}
Y.~Mao, M.~Szmuk, and B.~Acikmese, ``Successive convexification of non-convex
  optimal control problems and its convergence properties,'' in {\em 2016
  {{IEEE}} 55th {{Conference}} on {{Decision}} and {{Control}} ({{CDC}})},
  pp.~3636--3641, {IEEE}, Dec. 2016.

\bibitem{Camacho2007}
E.~F. Camacho and C.~Bordons, {\em Model Predictive Control}.
\newblock 2007.

\bibitem{Patterson2014a}
M.~A. Patterson and A.~V. Rao, ``{{GPOPS-II}}: {{A MATLAB Software}} for
  {{Solving Multiple-Phase Optimal Control Problems Using}} hp-{{Adaptive
  Gaussian Quadrature Collocation Methods}} and {{Sparse Nonlinear
  Programming}},'' {\em ACM Transactions on Mathematical Software}, vol.~41,
  pp.~1:1--1:37, Oct. 2014.

\bibitem{Kelley1962}
H.~J. Kelley, ``Method of {{Gradients}},'' in {\em Optimization {{Techniques
  With Applications}} to {{Aerospace Systems}}}, vol.~5, pp.~205--254,
  {Academic Press Inc.}, 1962.

\bibitem{DENHAM1964}
W.~F. DENHAM and A.~E. BRYSON, ``Optimal programming problems with inequality
  constraints. ii - solution by steepest-ascent,'' {\em AIAA Journal}, vol.~2,
  pp.~25--34, Jan. 1964.

\bibitem{Teo1989}
K.~L. Teo and L.~S. Jennings, ``Nonlinear optimal control problems with
  continuous state inequality constraints,'' {\em Journal of Optimization
  Theory and Applications}, vol.~63, pp.~1--22, Oct. 1989.

\bibitem{Han1979}
S.~P. Han and O.~L. Mangasarian, ``Exact penalty functions in nonlinear
  programming,'' {\em Mathematical Programming}, vol.~17, pp.~251--269, Dec.
  1979.

\bibitem{Hestenes1969}
M.~R. Hestenes, ``Multiplier and gradient methods,'' {\em Journal of
  Optimization Theory and Applications}, vol.~4, pp.~303--320, Nov. 1969.

\bibitem{BERTSEKAS1982a}
D.~P. BERTSEKAS, ``The {{Method}} of {{Multipliers}} for {{Inequality
  Constrained}} and {{Nondifferentiable Optimization Problems}},'' in {\em
  Constrained {{Optimization}} and {{Lagrange Multiplier Methods}}},
  pp.~158--178, {Elsevier}, 1982.

\bibitem{Jacobson1967}
D.~Jacobson and M.~Lele, ``A transformation technique for optimal control
  problems with a state variable inequality constraint,'' {\em IEEE
  Transactions on Automatic Control}, vol.~14, pp.~457--464, Oct. 1969.

\bibitem{Oguri2022d}
K.~Oguri and J.~W. McMahon, ``Stochastic {{Primer Vector}} for {{Robust
  Low-Thrust Trajectory Design Under Uncertainty}},'' {\em Journal of Guidance,
  Control, and Dynamics}, vol.~45, pp.~84--102, Jan. 2022.

\bibitem{Oguri2022a}
K.~Oguri and G.~Lantoine, ``Stochastic {{Sequential Convex Programming}} for
  {{Robust Low-thrust Trajectory Design}} under {{Uncertainty}},'' in {\em
  {{AAS}}/{{AIAA Astrodynamics Conference}}}, pp.~1--20, 2022.

\bibitem{Sidhoum2023a}
Y.~Sidhoum and K.~Oguri, ``Indirect {{Forward-Backward Shooting}} for
  {{Low-thrust Trajectory Optimization}} in {{Complex Dynamics}},'' in {\em
  {{AAS}}/{{AIAA Space Flight Mechanics Meeting}}}, p.~20, 2023.

\bibitem{Pontryagin1962}
L.~S. Pontryagin, V.~G. Boltyanskii, R.~V. Gamkrelidze, and E.~F. Mischenko,
  {\em The {{Mathematical Theory}} of {{Optimal Processes}}}.
\newblock {CRC Press}, 1962.

\bibitem{Bryson1963}
A.~E. Bryson, W.~F. Denham, and S.~E. Dreyfus, ``Optimal {{Programming
  Problems}} with {{Inequality Constraints I}}: {{Necessary Conditions}} for
  {{Extremal Solutions}},'' {\em AIAA Journal}, vol.~1, pp.~2544--2550, Nov.
  1963.

\bibitem{Conway2010}
B.~A. Conway, {\em Spacecraft {{Trajectory Optimization}}}.
\newblock {Cambridge}: {Cambridge University Press}, 2010.

\bibitem{Oguri2021d}
K.~Oguri and J.~W. McMahon, ``Stochastic {{Primer Vector}} for {{Robust
  Low-Thrust Trajectory Design Under Uncertainty}},'' {\em Journal of Guidance,
  Control, and Dynamics}, vol.~45, pp.~84--102, Jan. 2022.

\bibitem{Bonalli2022}
R.~Bonalli, T.~Lew, and M.~Pavone, ``Analysis of {{Theoretical}} and
  {{Numerical Properties}} of {{Sequential Convex Programming}} for
  {{Continuous-Time Optimal Control}},'' {\em IEEE Transactions on Automatic
  Control}, pp.~1--16, 2022.

\bibitem{Bonalli2019a}
R.~Bonalli, A.~Bylard, A.~Cauligi, T.~Lew, and M.~Pavone, ``Trajectory
  {{Optimization}} on {{Manifolds}}: {{A Theoretically-Guaranteed Embedded
  Sequential Convex Programming Approach}},'' in {\em Proceedings of
  {{Robotics}}: {{Science}} and {{Systems}}}, May 2019.

\bibitem{Oguri2019b}
K.~Oguri, M.~Ono, and J.~W. McMahon, ``Convex {{Optimization}} over
  {{Sequential Linear Feedback Policies}} with {{Continuous-time Chance
  Constraints}},'' in {\em 2019 {{IEEE}} 58th {{Conference}} on {{Decision}}
  and {{Control}} ({{CDC}})}, pp.~6325--6331, Dec. 2019.

\bibitem{Cesari1983}
L.~Cesari, ``Lagrange and {{Bolza Problems}} of {{Optimal Control}} and {{Other
  Problems}},'' in {\em Optimization\textemdash{{Theory}} and
  {{Applications}}}, vol.~10, pp.~196--205, {New York, NY}: {Springer New
  York}, 1983.

\bibitem{McINTYRE1967}
{\relax JOHN}.~McINTYRE and {\relax BERNARD}.~PAIEWONSKY, ``On {{Optimal
  Control}} with {{Bounded State Variables}},'' in {\em Advances in {{Control
  Systems}}}, vol.~5, pp.~389--419, {Elsevier}, 1967.

\bibitem{Taylor1972}
J.~Taylor, ``Comments on a multiplier condition for problems with state
  variable inequality constraints,'' {\em IEEE Transactions on Automatic
  Control}, vol.~17, pp.~743--744, Oct. 1972.

\bibitem{Taheri2018}
E.~Taheri and J.~L. Junkins, ``Generic {{Smoothing}} for {{Optimal
  Bang-Off-Bang Spacecraft Maneuvers}},'' {\em Journal of Guidance, Control,
  and Dynamics}, vol.~41, pp.~2470--2475, Nov. 2018.

\end{thebibliography}

